Sampling Efficient Deep Reinforcement Learning through Preference-Guided Stochastic Exploration

Massive practical works addressed by Deep Q-network (DQN) algorithm have indicated that stochastic policy, despite its simplicity, is the most frequently used exploration approach. However, most existing stochastic exploration approaches either explore new actions heuristically regardless of Q-values or inevitably introduce bias into the learning process to couple the sampling with Q-values. In this paper, we propose a novel preference-guided $\epsilon$-greedy exploration algorithm that can efficiently learn the action distribution in line with the landscape of Q-values for DQN without introducing additional bias. Specifically, we design a dual architecture consisting of two branches, one of which is a copy of DQN, namely the Q-branch. The other branch, which we call the preference branch, learns the action preference that the DQN implicit follows. We theoretically prove that the policy improvement theorem holds for the preference-guided $\epsilon$-greedy policy and experimentally show that the inferred action preference distribution aligns with the landscape of corresponding Q-values. Consequently, preference-guided $\epsilon$-greedy exploration motivates the DQN agent to take diverse actions, i.e., actions with larger Q-values can be sampled more frequently whereas actions with smaller Q-values still have a chance to be explored, thus encouraging the exploration. We assess the proposed method with four well-known DQN variants in nine different environments. Extensive results confirm the superiority of our proposed method in terms of performance and convergence speed. Index Terms- Preference-guided exploration, stochastic policy, data efficiency, deep reinforcement learning, deep Q-learning.

==> experiments/ablation.tex <==
\begin{figure}[!t]
\centering
    \hspace{0.3cm}\includegraphics[width=0.445\textwidth, height=0.2in]{photo/legend_v2.pdf}\\
    \subfigure[Alien]{\includegraphics[width=.24\textwidth]{photo/ablation_alien.pdf}\label{ablation:a}}
    \subfigure[Amidar]{\includegraphics[width=.24\textwidth]{photo/ablation_amidar.pdf}\label{ablation:b}}
\captionsetup{labelfont=bf}
\caption{Ablation study for embedding network sharing. ``PGDQN with $\epsilon$-greedy policy'': the modified PGDQN with $\epsilon$-greedy policy for sampling actions.}
\label{fig5}
\end{figure}

==> experiments/hyper-parameter.tex <==
\begin{table}[htbp]
\tiny
% increase table row spacing, adjust to taste
%\renewcommand{\arraystretch}{1.3}
%if using array.sty, it might be a good idea to tweak the value of
%\extrarowheight as needed to properly center the text within the cells
\caption{Hyper-parameter Settings for baselines and PGDQN.}
\begin{adjustbox}{width=0.5\textwidth,center}
\centering
% Some packages, such as MDW tools, offer better commands for making tables
% than the plain LaTeX2e tabular which is used here.
\begin{tabular}{c c}
\hline
% \multicolumn{0}{c}{Parameter}
% &\multicolumn{1}{c}{Value}\\
Parameter & Value\\
\hline
minibatch size & 32\\
reply buffer size & 1000000\\
learning start size & 50000\\
discount factor & 0.99\\
agent history length & 4\\
action repeat & 4\\
preference branch update frequency & 4\\
Q branch update frequency & 4\\
target network update frequency & 10000\\
RMSProp learning rate for preference-branch & 0.00025\\
RMSProp learning rate for Q-branch & 0.00025\\
RMSProp learning rate for baselines & 0.00025\\
Adam learning rate for temperature parameter & 0.00025\\
initial exploration & 1\\
final exploration & 0.1\\
final exploraiton frame & 1000000\\
\hline
\end{tabular}
\end{adjustbox}
\label{table3}
\end{table}

\begin{table}[H]
\vspace{-2cm}
\tiny
% increase table row spacing, adjust to taste
%\renewcommand{\arraystretch}{1.3}
%if using array.sty, it might be a good idea to tweak the value of
%\extrarowheight as needed to properly center the text within the cells
\caption{Architectures for baselines and PGDQN. All the algorithms utilize the CNN networks consisting of three hidden layers.}
\begin{adjustbox}{width=0.5\textwidth,center}
\centering
% Some packages, such as MDW tools, offer better commands for making tables
% than the plain LaTeX2e tabular which is used here.
\begin{tabular}{c c}
\hline
% \multicolumn{0}{c}{Parameter}
% &\multicolumn{1}{c}{Value}\\
Parameter & Value\\
\hline
input dimension & [84, 84, 4]\\
first hidden layer & [4, 32]\\ 
kernel size & 8 $\times$ 8\\
stride size & 4\\
second hidden layer & [32, 64]\\
kernel size & 4 $\times$ 4\\
stride size & 2\\
third hidden layer & [64, 64]\\
kernel size & 3 $\times$ 3\\
stride size & 1\\
latent state space dimension & [7, 7, 64]\\
fully connected layer for Q-branch & 256\\
fully connected layer for preference branch & 256\\
fully connected layer for baselines & 512\\
output dimension & $dim(\mathcal{A})$\\
\hline
\end{tabular}
\end{adjustbox}
\label{table4}
\end{table}
